Tests of the Quark-Gluon Plasma Coupling Strength at Early Times with Heavy Quarks

The redistribution in momentum space of heavy quarks via their interactions in the quark-gluon plasma is an excellent probe of the heavy quark coupling strength to the medium. We utilize a Monte Carlo Langevin calculation for tracking heavy quark - antiquark pairs embedded in a viscous hydrodynamic space-time evolution. We find that the nuclear modification factor ($R_{AA}$) for charm quarks is relatively insensitive to the coupling to the quark-gluon plasma at early times where the highest temperatures are acheived. In contrast the azimuthal angular correlation of charm and anticharm quarks is extremely sensitive to the early time evolution. For beauty quarks the situation is reversed in terms of sensitivity. Future measurements of heavy quarks have the potential to map out the temperature dependence of the shear viscosity to entropy density ratio ({\eta}/s).

==> Makefile <==
FILENAME=main

TEXSDIR = ./
FIGSDIR = ./figs
TEXSRCS = $(shell find $(TEXSDIR) -maxdepth 1 -iname "*.tex")
FIGS    = $(shell find $(FIGSDIR) -maxdepth 1 -iname "*.pdf") #TODO add .jpg, etc.
ADDFILES= Makefile langevin.bib
PDFTEX  = pdflatex # Select pdflatex or xelatex
BIBTEX  = bibtex

default: $(FILENAME).pdf

$(FILENAME): $(FILENAME).dvi

$(FILENAME).pdf: $(FILENAME).tex $(TEXSRCS) $(FIGS) $(ADDFILES)
	$(PDFTEX) $(FILENAME)
	$(BIBTEX) $(FILENAME)||true
	$(PDFTEX) $(FILENAME)
	$(PDFTEX) $(FILENAME)

open:
	open ${FILENAME}.pdf

clean:
	rm -f \
	*.log \
	*.aux \
	*.out \
	*.dvi \
	*.bbl \
	*.blg \
	*.nav \
	*.snm \
	*.toc

.phony: clean open

